Thingi10K: A Dataset of 10,000 3D-Printing Models

Empirically validating new 3D-printing related algorithms and implementations requires testing data representative of inputs encountered \emph{in the wild}. An ideal benchmarking dataset should not only draw from the same distribution of shapes people print in terms of class (e.g., toys, mechanisms, jewelry), representation type (e.g., triangle soup meshes) and complexity (e.g., number of facets), but should also capture problems and artifacts endemic to 3D printing models (e.g., self-intersections, non-manifoldness). We observe that the contextual and geometric characteristics of 3D printing models differ significantly from those used for computer graphics applications, not to mention standard models (e.g., Stanford bunny, Armadillo, Fertility). We present a new dataset of 10,000 models collected from an online 3D printing model-sharing database. Via analysis of both geometric (e.g., triangle aspect ratios, manifoldness) and contextual (e.g., licenses, tags, classes) characteristics, we demonstrate that this dataset represents a more concise summary of real-world models used for 3D printing compared to existing datasets. To facilitate future research endeavors, we also present an online query interface to select subsets of the dataset according to project-specific characteristics. The complete dataset and per-model statistical data are freely available to the public.

==> motivation.tex <==

\section{Motivation}
\label{sec:motivation}

Just like any emerging technologies, 3D printing faces a number of challenges
that prevent it from scaling up and expanding into new markets.
Computational fabrication research community has tackled a number of such
challenges over the years,
include predicting structural weakness (\cite{Stava:2012,Zhou2013,Umetani:2013}),
computational design to reduce material cost without compromising structure strength
(\cite{Wang:2013,Lu:2014}),
%designing microstructure to achieve given deformation
%(\cite{Panetta:2015,Schumacher:2015}),
or take a given pose under gravity (\cite{Chen:2014}),
structural optimization to ensure a shape is balanced (\cite{Prevost:2013}),
spin-able (\cite{Bacher:2014}), or other behaviors (\cite{Musialski:2015}).

While these works solves very different problems, they all share the common
assumption that input 3D mesh is clean
so that simulation and geometric optimization can be carried out.
However, as we will show in this paper, such assumption is often false.
3D shapes designed for fabrication often contain degeneracies, overlapping
faces and self-intersections.
Such problems with input meshes are major blocks that limits
the applicability of computational fabrication algorithms to the real world.

In this work, we take the first step towards understanding the nature of 3D
printed shapes used in practice.  By documenting both contextual and geometric
information of 10,000 3D printing models, we hope to achieve the following
goals:

% Stress test dataset support filtering on geometry and contextual data.
% Evaluates the restriction of common preconditions.
% Provide a large scale annotated 3D dataset for learning semantics from
% geometry.
%

\begin{itemize}
\item Quantitatively analyze ``issues'' of real-world 3D models for fabrication purposes.
\item Provide a query interface to select models based on contextual and
geometric criteria.
\item Provide a large scale annotated dataset for training machine learning
algorithms.
\end{itemize}

%Why wild model matters.

%Interesting things we can do with this dataset.



==> related.tex <==

\section{Related Works}
\label{sec:related}

One major factor for the abundance of 3D models today is the continuous efforts
of computer graphics research community.
Many authors, such as \cite{sumner2004}, released 3D examples used in their work
to the general public.
Another source of models is specialized dataset designed for specific
applications such as the IKEA dataset by \cite{lpt2013ikea}.
While surveying all public 3D dataset is beyond the goal of
this work, in this section, we summarize existing large scale dataset that share
similar goals with ours.

Perhaps the most well-known model repository is The Stanford 3D Scanning
Repository (\cite{levoy2005}).  It consists of 9 high resolution models
originating from range scans.  All models are manifold and degeneracy-free,
which make them ideal as proof-of-concept examples.  These models are released
in ASCII PLY format.

The Princeton Shape Benchmark (\cite{shilane2004}), another popular 3D model
dataset, consists of 1,814 polygonal models collected from the World Wide Web in
2004. It includes low resolution models of a variety of real world objects.
Version 1 of the dataset is designed for training 3D classification algorithms.
It is divided into a training set of 907 models and a testing set of 907 models.
Each model is accompanied by a classification file that specifies its
functionality.
All models in this dataset are encoded in ASCII OFF format.

For the last 10 years, Shape Retrieval Contest has released
multiple datasets each year to test algorithms ranging from 
generic or large scale shape retrieval
(\cite{li2012shrec,bronstein2010shreclarge}),
non-rigid human model retrieval (\cite{pickup2014shrec}),
sketch-based shape retrieval (\cite{li2013shrec,li2014shrec}),
shape correspondence (\cite{bronstein2010shrec}),
facial model retrieval (\cite{nair2008shrec,veltkamp2011shrec}),
range scan retrieval (\cite{dutagaci2010shrec}),
 etc.
Each dataset typically focus on a single data type (e.g. range scan) from a
common data source; its models may be sampled from a existing dataset,
modified based on existing models or
collected consistently with specific techniques.

Recently, \cite{shapenet2015} introduced ShapeNet, a large scale 3D dataset
consisting of more than 3,000,000 CAD models retrieved from
2 online shape
repositories: Trimble 3D Warehouse and Yobi3D. Using a semi-automatic annotation
methodology, the majority of models are tagged with semantic information.
Because ShapeNet is designed for
machine learning purposes, it prefers clean and
high quality models that are easy to use.  Its subset, ShapeNetCore, only
contains models made of single connected component.  In addition, because models
are retrieved via textual queries, the categories of the models are somewhat
biased by human selection.

More recently, \cite{Beyer:2015} uses 2,250 3D models from Thingiverse
to test their Platener algorithm.
\cite{Choi2016} released a large dataset consisting of more than
10,000 object scan data, based on which, 398 3D reconstructions were created and
released.

While our dataset are not the first 3D shape dataset proposed, it is different
with datasets aforementioned in several key aspect.

\begin{description}

\item{\textbf{Quantity}}: With the exception of \cite{shapenet2015}, our dataset
contains more 3D models than all previous datasets.
\item{\textbf{Purpose}}: To the best of our knowledge, our work is the first large
scale study on 3D shape for fabricate purposes.
All models in our dataset are designed to be 3D printed, and
most of them are physically fabricated by one or more Thingiverse users.
\item{\textbf{Intact}}: Our dataset reflects the raw state of 3D printed
shapes without any deliberate filtering or modification by us.
\item{\textbf{Annotated}}: Each model in our dataset are annotated with information
on category, subcategory and a number of textual tags.
All annotations are created by the original authors of each model.
\item{\textbf{Diverse sources}}:
Models in our dataset are created by thousands of individual designers with
different backgrounds and skills.
\item{\textbf{Query support}}: Similar to \cite{shapenet2015}, we release a web interface that
allow users to easily browse models in our dataset.  In addition, our web interface
supports textual queries on both contextual and geometric properties.  See
section \ref{sec:interface} for details.
\end{description}



